A Hierarchical Slice Attention Network for Appendicitis Classification in 3D CT Scans

Timely and accurate diagnosis of appendicitis is critical in clinical settings to prevent serious complications. While CT imaging remains the standard diagnostic tool, the growing number of cases can overwhelm radiologists, potentially causing delays. In this paper, we propose a deep learning model that leverages 3D CT scans for appendicitis classification, incorporating Slice Attention mechanisms guided by external 2D datasets to enhance small lesion detection. Additionally, we introduce a hierarchical classification framework using pre-trained 2D models to differentiate between simple and complicated appendicitis. Our approach improves AUC by 3% for appendicitis and 5.9% for complicated appendicitis, offering a more efficient and reliable diagnostic solution compared to previous work.

==> img/overview.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[scale=0.30]{img/overview.png}
    \caption{(a), (b) and (c) are the CC, NSS, KLD score of IFCB map of the three datasets respectively. (d) is an illustration of equation  The slope of the curve becomes steeper as alpha increases.}
    \label{overview}
\end{figure*}

==> table/Datasets.tex <==
% \documentclass{article}
% \usepackage{graphicx}

% \begin{document}

% \section*{Datasets}

% \subsection*{NTUH datasets}
% \usepackage{float}

% \begin{table}[t]
% \centering
%     \begin{tabular}{|l|c|c|c|c|}
%     \hline
%     \textbf{Set} & \textbf{Total} & \textbf{Appendicitis} & \textbf{\makecell{Perforation}} & \textbf{\makecell{Abscess}} \\
%     \hline
%     train & 1715 & 689 & 107 & 65 \\
%     \hline
%     val & 216 & 89 & 13 & 8 \\
%     \hline
%     test & 226 & 89 & 14 & 9 \\
%     \hline
%     \end{tabular}
% \caption{NTUH datasets}
% \end{table}

% % \subsection*{FEMH datasets}
% \begin{table}[t]
% \centering
%     \begin{tabular}{|l|c|c|c|c|}
%     \hline
%     \textbf{Set} & \textbf{Total} & \textbf{Appendicitis} & \textbf{\makecell{Perforation}} & \textbf{\makecell{Abscess}} \\
%     \hline
%     train & 624 & 535 & 81 & 43 \\
%     \hline
%     val & 218 & 189 & 31 & 19 \\
%     \hline
%     test & 214 & 184 & 31 & 15 \\
%     \hline
%     \end{tabular}
% \caption{FEMH datasets}
% \end{table}
\begin{table}[t]
\centering
    \begin{tabular}{|l|c|c|c|c|}
    \hline
    \textbf{Set} & \textbf{Total} & \textbf{Appendicitis} & \textbf{\makecell{Perforation}} & \textbf{\makecell{Abscess}} \\
    \hline
    train & 2339 & 1224 & 188 & 108 \\
    \hline
    val & 434 & 278 & 44 & 27 \\
    \hline
    test & 440 & 273 & 45 & 24 \\
    \hline
    \end{tabular}
\caption{Combined NTUH and FEMH datasets}
\end{table}

% \end{document}


==> table/NTUH.tex <==
\begin{table*}[b]
	\centering
	\caption{Model accuracy improved after applying CAMIM pretraining on a subset of the NTUH dataset. This subset was manually selected to include challenging cases.} 
    \vspace*{5mm}
	\begin{tabular}{|c|c|c|c|c|c|c|c|}
        \hline
        Lesion & Model & AUC & ACC & F1-score & Sensitivity &
Specificity & Precision \\
		\hline
  		Appendicitis 
        & Avg. Perf. of Manual Interpretation & . & 0.602 & 0.559 & 0.840 & 0.500 & 0.419  \\
        \cline{2-8}
		& AppendixNet \cite{rajpurkar2020appendixnet} & . & 0.740 & 0.667 & . & . & .  \\
        \cline{2-8}
        & 3D Resnet & . & . & . & . & . & . \\
        \cline{2-8}
        & CNN-base \cite{park2020convolutional}& . & . & . & . & . & . \\
        \cline{2-8}
        & RGB-EfficientNet \cite{park2023comparison} & . & . & . & . & .& .\\
        \cline{2-8}
        & Fusion Model (ours model) & 0.788 &  0.7 &  0.651 & 0.824 & 0.636 & 0.538  \\
		\hline
         \hline
		% Appendicolith & Avg. Perf. of Manual Interpretation & . & . &. & . & .   \\
  %       \cline{2-7}
		%               & AppendixNet & . & . & . & . & . \\
  %       \cline{2-7}
  %                                & 3D Resnet & . & . & . & . & .\\
  %       \cline{2-7}
  %                                & CNN-base & . & . & . & . & .\\
  %       \cline{2-7}
  %                                & RGB-EfficientNet & . & . & . & . & .\\
  %       \cline{2-7}
  %                             & Fusion Model (ours model) & . & . &. & . & . \\
		% \hline
  		Perforation 
        & Avg. Perf. of Manual Interpretation & . & 0.826 & 0.243 & 0.350 & 0.867 & 0.187  \\
        \cline{2-8}
		& AppendixNet \cite{rajpurkar2020appendixnet} & . & . &. & . & . & .  \\
        \cline{2-8}
        % & 3D Resnet & . & . & . & . & . & . \\
        % \cline{2-8}
        % & CNN-base \cite{park2020convolutional} & . & . & . & . & . & . \\
        % \cline{2-8}
        % & RGB-EfficientNet \cite{park2023comparison} & . & . & . & . & .& .\\
        % \cline{2-8}
        & Fusion Model (ours model) & 0.716 &  0.8 &  0.375 & 0.6 & 0.822 & 0.273  \\
		\hline
        \hline
  		Abscess 
        & Avg. Perf. of Manual Interpretation & . & 0.810 & 0.264 & 0.567 & 0.826 & 0.172  \\
        \cline{2-8}
	    & AppendixNet \cite{rajpurkar2020appendixnet} & . & . &. & . & . & .  \\
        \cline{2-8}
        % & 3D Resnet & . & . & . & . & . & . \\
        % \cline{2-8}
        % & CNN-base \cite{park2020convolutional}& . & . & . & . & . & . \\
        % \cline{2-8}
        % & RGB-EfficientNet \cite{park2023comparison} & . & . & . & . & .& .\\
        % \cline{2-8}
        & Fusion Model (ours model) & 0.787 &  0.9 & 0.286 & 0.333 & 0.936 & 0.25  \\
		\hline
     \end{tabular}
     \label{table:NTUH}
\end{table*}



==> tex/2_related_works.tex <==
\section{Related Works}
\label{sec:Related Works}
\subsection{Abdomen CT Imaging Classification}
Recent advancements in deep learning have significantly impacted the classification of abdominal CT images for diagnosing appendicitis. Park et al. (2020) \cite{park2020convolutional} explored a CNN-based diagnostic algorithm for appendicitis using CT scans from patients with acute abdominal pain. AppendiXNet \cite{rajpurkar2020appendixnet}, a 3D deep learning model, utilizes video pretraining to effectively address the challenge of small medical datasets. Park et al. (2023) \cite{park2023comparison} investigated the use of EfficientNet for classifying acute appendicitis, acute right-sided diverticulitis, and normal appendix from CT images. Their research compared the effectiveness of single versus serial CT imaging, finding that serial imaging provided better diagnostic performance. In our work, we propose a hybrid 2D-3D fusion model that leverages pre-trained 2D models and integrates external 2D information to enhance 3D CT image classification. 
\subsection{Slice Importance Detection in 3D Imaging}
Accurately identifying the most relevant slices in 3D imaging is crucial for effective diagnosis. Several studies have focused on this challenge. \cite{bai2023representative} Chen et al. (2022) presented a technique for identifying infectious slices in pulmonary tuberculosis CT scans through representative slice selection and multi-view projection learning, enhancing diagnostic accuracy by focusing on key slices. \cite{wang2022key} Wang et al. (2022) proposed a supervised Key-frame Guided Network for thyroid nodule recognition, utilizing a detection-localization framework and motion attention to focus on significant frames. \cite{li2022satr}Li et al. (2022) introduced the Slice Attention Transformer (SATr), which enhances lesion detection in CT scans by modeling long-distance dependencies within and across slices using a transformer-based approach. \cite{sun2023boosting} Sun et al. (2023) developed a self-supervised method for breast ultrasound video classification that uses keyframe feature centers to guide frame attention, improving classification performance without needing explicit keyframe labels. However, in many scenarios, such as ours, where labels for key slices are not available, self-supervised methods become essential. Motivated by Sun et al. (2023), we adopt a self-supervised approach to tackle this challenge, enhancing the detection and classification of appendicitis and related lesions in 3D CT images.

\subsection{Hybrid 2D-3D Fusion Models}
Hybrid 2D-3D fusion models have emerged as a promising solution to leverage the strengths of both 2D and 3D data in medical image analysis. \cite{roy2019hybridsn} Roy et al. (2020) introduced HybridSN, which combines 3D and 2D convolutions to balance spatial-spectral feature extraction in hyperspectral image classification, reducing computational complexity while enhancing performance. \cite{jang2022m3t} Jang and Hwang (2022) developed M3T, a three-dimensional medical image classifier that synergizes 3D CNN, 2D CNN, and transformer architectures for accurate Alzheimer's disease classification from MRI scans. This approach utilizes 2D CNNs for pre-trained weight leverage and transformers for capturing long-range dependencies, demonstrating the efficacy of hybrid models in medical imaging. Inspired by these methods, our work employs a hybrid 2D-3D fusion model to address the scarcity of 3D abdominal CT data and enhance the classification of appendicitis and related lesions by integrating pre-trained 2D models with 3D spatial information.

